TOP: Towards Open & Predictable Heterogeneous SoCs

Ensuring predictability in modern real-time Systems-on-Chip (SoCs) is an increasingly critical concern for many application domains such as automotive, robotics, and industrial automation. An effective approach involves the modeling and development of hardware components, such as interconnects and shared memory resources, to evaluate or enforce their deterministic behavior. Unfortunately, these IPs are often closed-source, and these studies are limited to the single modules that must later be integrated with third-party IPs in more complex SoCs, hindering the precision and scope of modeling and compromising the overall predictability. With the coming-of-age of open-source instruction set architectures (RISC-V) and hardware, major opportunities for changing this status quo are emerging. This study introduces an innovative methodology for modeling and analyzing State-of-the-Art (SoA) open-source SoCs for low-power cyber-physical systems. Our approach models and analyzes the entire set of open-source IPs within these SoCs and then provides a comprehensive analysis of the entire architecture. We validate this methodology on a sample heterogenous low-power RISC-V architecture through RTL simulation and FPGA implementation, minimizing pessimism in bounding the service time of transactions crossing the architecture between 28% and 1%, which is considerably lower when compared to similar SoA works.

==> ANALYSIS/lemma2_modified.tex <==
\begin{lemma}\label{lemma:max_num_intf_read}
    \review{Let $C_i$ issues $V \leq \phi_X^{C_i}$ transactions, with $AX_{i,j}$ being the $V^{th}$.}
    %
    \review{The maximum number of transactions of the same type that can interfere with $AX_{i,j}$ is upper bounded by:}
    %
    \begin{equation}\label{read_with_read}
    \footnotesize
    S^{X}_{i,j} = min\left(V - 1 + \sum_{C_y \in \Psi_j} \phi_X^{C_y} , V - 1 + \chi_X^{P_j} + V \cdot \bigm|\Psi_j\bigm| \right)
    \end{equation}
    \begin{equation}\label{read_with_read}
    \footnotesize
    S^{X}_{i,j} = min\left(\sum_{C_y \in \Psi_j} \phi_X^{C_y} , \chi_X^{P_j} + \phi_X^{C_i} \cdot \bigm|\Psi_j\bigm| \right)
    \end{equation}
\end{lemma}

\begin{proof}
    The $\min$ in the formula has two components.
    %
    An interfering \emph{controller} $C_k$ cannot have more than $\phi_{X}^{C_k}$ pending outstanding transactions.
    %
    \review{Hence, the maximum number of transactions issued by the \emph{controllers} in $\Psi_j$ that can interfere with $AX_{i,j}$ is bound by $\sum_{C_y \in \Psi_j} \phi_X^{C_y}$.}
    %
    \review{The number of transactions issued by $C_i$ preceding $AX_{i,j}$ is equal to $V - 1$.}
    %
    \review{Summing these two contributions provides an upper bound on the number of transactions of the same type interfering with $AX_{i,j}$ -- the left member of the $\min$ derives.}
    %
    From our \emph{peripheral} analysis reported in Section~\ref{sec:wcea}, $P_j$ and $R_0$ can limit the maximum amount of transactions accepted by the system: $P_j$ accepts overall at most $\chi_{R/W}^{P_j}$ transactions -- when such a limit is reached, any further incoming transaction directed to $P_j$ is stalled.
    %
    After $P_j$ serves a transaction, $R_0$ restarts forwarding transactions to the \emph{peripheral} following a round-robin scheme (see Section~\ref{sec:wcea}).
    %
    In the worst-case scenario, $C_i$ loses the round-robin arbitration against all of the $\bigm|\Psi_j\bigm|$ interfering \emph{controllers} in $\Psi_j$.
    %
    \review{Once the first arbitration is lost, this applies to all the $V-1$ transactions preceding $AX_{i,j}$, and to $AX_{i,j}$ as well.}
    %
    \review{Therefore, $V \cdot \bigm|\Psi_j\bigm|$ safely bounds the number of transactions that can precede $AX_{i,j}$ because of the contention.}
    %
    \review{Summing up these two contributions, together with $V-1$ as done before, also $ V -1 + \chi_{R}^{P_j} + V \cdot \bigm|\Psi_j\bigm|$ upper bounds the maximum number of transactions interfering with $AX_{i,j}$ -- the right member of the $\min$ derives.}
    %
    Both of the bounds are valid -- the minimum between them is an upper bound providing the least pessimism -- Lemma \ref{lemma:max_num_intf_read} derives.
\end{proof}

==> todo.tex <==
TODO:

1. Additional bound on the SPM at system level, to consider the parallelism.

\begin{equation}\label{eq:max_intf_1trx}
     l_{R/W}^{AX_{i,j}} = t_{\text{CTRL,R/W}}^{P_j} + t_{\text{DATA,R/W}}^{P_j} \cdot \beta + d_{\text{R/W}}^{R_0}
\end{equation}
\begin{equation}\label{eq:max_intf_1trx}
     l_{R/W}^{AX_{i,j}} = t_{\text{DATA,R/W}}^{P_j} \cdot \beta + d_{\text{R/W}}^{R_0}
\end{equation}
